Neutrino-(anti)neutrino forward scattering potential for massive neutrinos at low energies

In this work, we calculate expression for the potential due to neutrino-(anti)neutrino forward scattering at low energies ($E<<m_{Z^0}$) for ultra-relativistic massive neutrinos ($E>>m_{\nu}$), a representative regime within astrophysical scenarios. There is a broadly used expression for this potential in the literature, which, however, lacks an explicit derivation from basic principles of quantum field theory. Therefore, this paper has the intention to guide the reader through the steps and concepts to derive this potential, trying to be clear and pedagogical. Moreover, we used a rigorous approach concerning the massive nature of the neutrinos, using massive quantized neutrino fields throughout the entire process, while the usual approach is to consider massless neutrino fields at the interaction. In this context, we explicitly show the validity of the massless neutrino fields approximation at the ultra-relativistic regime, as expected. As the last step, we connect the potential expression to the density matrix formalism, which is a usual framework for works considering neutrino-neutrino interactions. We also discuss some theoretical details through the paper, such as the normal ordering of quantum operators and the implications of massive fields in the neutrino state at its production.

==> Neutrino-Neutrino Potential_Massive Fields_Arxiv/Conventions.tex <==
Here we describe our conventions regarding the neutrinos quantized fields and states. We take the following Fourier expansion for the quantized neutrino fields, using a finite normalization volume $V$ with periodic conditions,

\begin{equation}
\label{eq:field_expansion_V}
\begin{split}
        \nu_\alpha(x)&= \sum_{\vec{p},s}  \frac{1}{\sqrt{2VE_{\vec{p}}}} \left [ a^s_{\vec{p}} u^s(\vec{p}) e^{-ipx} +  b^{s \dagger}_{\vec{p}} v^s(\vec{p}) e^{ipx}\right ]
\end{split}
\end{equation}

\begin{equation}
\label{eq:field_expansion_adj_V}
\begin{split}
        \overline{\nu}_\alpha(x)&= \sum_{\vec{p}, s}  \frac{1}{\sqrt{2VE_{\vec{p}}}} \left [ a^{s \dagger}_{\vec{p}} \overline{u}^s(\vec{p}) e^{ipx} +  b^{s}_{\vec{p}} \overline{v}^s(\vec{p}) e^{-ipx}\right ]
\end{split}
\end{equation}

where the anti-commutation relations are
\begin{equation}
    \{  a^{s \dagger}_{p},  a^{s' \dagger}_{p'} \} = \{  b^{s \dagger}_{p},  b^{s' \dagger}_{p'} \} =\delta_{\vec{p}\vec{p}'} \delta_{ss'}
\end{equation}

Therefore, the fields obey the canonical equal-time anticommutation rules

\begin{equation}
    \{ \nu_\alpha (t,\vec{x}), \nu^{\dagger}_\beta (t,\vec{y}) \} = \delta^{(3)} (\vec{x} - \vec{y}) \delta_{\alpha \beta}
\end{equation}

The one particle states are defined as
\begin{equation}
    \ket{\nu(p,s)}=  a^{s \dagger}_{\vec{p}} \ket{0}   \text{,} \;\;\;\;\;  \ket{\overline{\nu}(p,s)}=  b^{s \dagger}_{\vec{p}} \ket{0}
\end{equation}

where their normalization is given by
\begin{equation}
    \bra{\nu(p,s)}\ket{\nu(p',s')} =  \bra{\overline{\nu}(p,s)}\ket{\overline{\nu}(p',s')} = \delta_{\vec{p}\vec{p}'} \delta_{ss'}
\end{equation}

Note that for Majorana neutrinos $a^{s \dagger}_{p}=b^{s \dagger}_{p}$. 



==> Neutrino-Neutrino Potential_Massive Fields_Arxiv/Potential_Normalization.tex <==
The one-particle states of momentum $\vec{p}$ are defined in a way that their normalization is Lorentz invariant. 

\begin{equation}
\label{eq:B_normaliztion}
    \bra{\vec{q}}\ket{\vec{p}} = (2\pi)^3 2E_{\vec{p}} \delta^{(3)} (\vec{p}-\vec{q})
\end{equation}

However, as in quantum mechanics, these states are not properly normalized to one in the continuum regime, and therefore can not describe physical particles. One way to get rid of this is to use wave packets properly normalized to represent particles. Another way is to consider finite volume normalization with periodic boundary conditions. That shows us that amplitudes calculated using states such as in \ref{eq:B_normaliztion} will not be properly normalized. However, the right normalization using these states can be achieved by the following process.

\begin{equation}
    \mathcal{A}_{norm} = \frac{\mathcal{A}_{fi}}{\sqrt{\bra{f}\ket{f}\bra{i}\ket{i}}}= \frac{\mathcal{A}_{fi}}{\prod_{i}^{} \sqrt{E_i} \prod_{f}^{} \sqrt{E_f}} = \frac{\bra{f}\mathcal{S}\ket{i}}{\sqrt{\bra{f}\ket{f}\bra{i}\ket{i}}}
\end{equation}


==> Neutrino-Neutrino Potential_Massive Fields_Arxiv/Trace_Techniques.tex <==
Here we derived some properties of spinors and Dirac matrices that are useful to our work. The resulting properties may be found by the name of "trace techniques" in the literature, as they translate the product of spinors and Dirac matrices into trace expressions.

\subsection{Spinor to Trace}

Lets consider a spinor that obeys the Dirac equation

\begin{equation}
    (\not{p} - m) u^{(h)}(p) = 0
\end{equation}
\begin{equation}
    \overline{u}^{(h)}(p) (\not{p} - m) = 0
\end{equation}

The helicity projector can be written as

\begin{equation}
    P_{h} = \frac{1+\gamma^{5}\not{s}_{h}}{2}
\end{equation}

where

\begin{equation}
    s^{\mu}_{h} = h \left( \frac{|\vec{p}|}{m} , \frac{E}{m} \frac{\vec{p}}{|\vec{p}|}\right)
\end{equation}

 Also, lets consider the completeness relation

\begin{equation}
\label{eq:spinor_completeness}
    \sum_{h=1}^{2} u^{h}(p) \overline{u}^{h}(p) = P_{h=1} u^{h}(p) \overline{u}^{h}(p) + P_{h=2} u^{h}(p) \overline{u}^{h}(p) = \not{p}+m
\end{equation}
Note that this expression is a $4\times4$ matrix, which can be seen due to the Dirac matrix in $\not{p}=\gamma^{\mu}p_{\mu}$. In general, all the vertices factors in SM interactions can be written as $ \overline{u}^{h}(p) \Gamma  u^{h}(p)$ where $\Gamma$ is a combination of Dirac matrices. We can use the relations above to turn this interaction factor into a trace expression.

\begin{equation}
\begin{split}
\label{eq:trace_projection}
    \overline{u}^{(h)}(p) \Gamma  u^{(h)}(p) =& \sum_{m,n}  \overline{u}^{(h)}_{n}(p) \Gamma_{nm}  u^{(h)}_{m}(p) = \sum_{m,n}   u^{(h)}_{m}(p) \overline{u}^{(h)}_{n}(p) \Gamma_{nm} \\
    =& \sum_{m,n}  \left[ P_{h} (\not{p}+m) \right]_{mn} \Gamma_{nm} = \sum_{m}\left[ P_{h}  (\not{p}+m) \Gamma \right]_{mm} \\
    =& Tr\left[ P_{h} (\not{p}+m) \Gamma \right] = Tr\left[ \frac{1+\gamma^{5}\not{s}_{h}}{2} (\not{p}+m) \Gamma \right]\\
    =& Tr\left[ (\not{p}+m) \left(\frac{1+\gamma^{5}\not{s}_{h}}{2} \right) \Gamma \right] 
\end{split}
\end{equation}
 
 Note that going from the first line to the second, we have used only one helicity component of equation \ref{eq:spinor_completeness}. Note also that $[\gamma^{5}\not{s}_{h},\not{p}]=0$. In the same way, we can derive the following expression for the sum over the helicity states.
 
 \begin{equation}
 \label{eq:trace_sum}
    \sum_{h=1}^{2} \overline{u}^{(h)}(p) \Gamma  u^{(h)}(p) = Tr\left[ (\not{p}+m) \Gamma \right] 
 \end{equation}
 
 \subsection{Weak SM interactions}
In the specific case of weak interactions of the Standard Model, we have the following V-A structure $\Gamma= \gamma^{\mu}(1-\gamma^5)$. Therefore, equation \ref{eq:trace_projection} became 
 
\begin{equation}
\begin{split}
 \overline{u}^{(h)}(p) \gamma^{\mu}(1-\gamma^5)  u^{(h)}(p) =&  \frac{1}{2} Tr\left[(\not{p}+m) (1+\gamma^{5}\not{s}_{h}) \gamma^{\mu}(1-\gamma^5) \right]=\\
 =& \frac{1}{2} Tr[(\not{p}+m)(\gamma^{\mu}-\gamma^{\mu}\gamma^{5}+\gamma^{5}\not{s}_{h}\gamma^{\mu}-\gamma^{5}\not{s}_{h}\gamma^{\mu}\gamma^{5})]=\\
 =& \frac{p_{\nu}}{2} Tr[\gamma^{\nu}\gamma^{\mu}-\gamma^{\nu}\gamma^{\mu}\gamma^{5}+\gamma^{\nu}\gamma^{5}\gamma^{\sigma} s^{h}_{\sigma}\gamma^{\mu}-\gamma^{\nu}\gamma^{5}\gamma^{\sigma} s^{h}_{\sigma}\gamma^{\mu}\gamma^{5}]\\
  +& \frac{m}{2} Tr[\gamma^{\mu}-\gamma^{\mu}\gamma^{5}+\gamma^{5}\gamma^{\sigma} s^{h}_{\sigma}\gamma^{\mu}-\gamma^{5}\gamma^{\sigma} s^{h}_{\sigma}\gamma^{\mu}\gamma^{5}]
\end{split}
\end{equation}

Using the following proprieties\footnote{And the trace property $ Tr[A+B] = Tr[A] + Tr[B]$.}

\begin{equation}
\begin{split}
    &Tr[\gamma^{\nu}\gamma^{\mu}] = 4 g^{\mu\nu}\\
    &Tr[\gamma^{\nu}\gamma^{\mu}\gamma^{5}] = 0\\
    &Tr[\gamma^{\nu}\gamma^{5}\gamma^{\sigma}\gamma^{\mu}] = 0\\
    &Tr[\gamma^{\nu}\gamma^{5}\gamma^{\sigma}\gamma^{\mu}\gamma^{5}] = Tr[\gamma^{\nu}\gamma^{\sigma}\gamma^{\mu}]= 0\\
\end{split}
\end{equation}

\begin{equation}
\begin{split}
    &Tr[\gamma^{\mu}] = 0\\
    &Tr[\gamma^{\mu}\gamma^{5}] = 0\\
    &Tr[\gamma^{5}\gamma^{\sigma}\gamma^{5}] = 0\\
    &Tr[\gamma^{5}\gamma^{\sigma}\gamma^{\mu}\gamma^{5}] = Tr[\gamma^{\sigma}\gamma^{\mu}]= 4g^{\sigma\mu}\\
\end{split}
\end{equation}

we finally have our desired relation.

\begin{equation}
\label{eq:A_spinor_projection}
    \overline{u}^{(h)}(p) \gamma^{\mu}(1-\gamma^5)  u^{(h)}(p) = 2(p^{\mu} - m s^{\mu}_h)
\end{equation}

We can use the same reasoning for the equation \ref{eq:trace_sum} and obtain the relation bellow.

\begin{equation}
\label{eq:A_spinor_sum}
    \sum_{h=1}^2 \overline{u}^{(h)}(p) \gamma^{\mu}(1-\gamma^5)  u^{(h)}(p) = 4p^{\mu}
\end{equation}

